A Coloring Algorithm for Disambiguating Graph and Map Drawings

Drawings of non-planar graphs always result in edge crossings. When there are many edges crossing at small angles, it is often difficult to follow these edges, because of the multiple visual paths resulted from the crossings that slow down eye movements. In this paper we propose an algorithm that disambiguates the edges with automatic selection of distinctive colors. Our proposed algorithm computes a near optimal color assignment of a dual collision graph, using a novel branch-and-bound procedure applied to a space decomposition of the color gamut. We give examples demonstrating the effectiveness of this approach in clarifying drawings of real world graphs and maps.

==> lab.tex <==
\section{Color Spaces and color Palettes}


Up to this point we do not specify the color space, other than assuming that the color space is
continuous, and color
difference between two colors can be measured using Euclidean
distance in the color space.

\subsection{RGB color space}

An often used color model is RGB. This is a model which defines color
by a combination of three color intensities, red, green, and blue.
Thus colors in the RGB model can be considered as residing in a
three-dimensional space.  The choice of these three primary colors is
related to the fact that human eyes normally have three kinds of cones
(a type of photo-receptor cells). The L cones respond the most to long
wavelength, peaking at a reddish color of around $575 \mu m$. The M
cones respond the most to medium wavelength, peaking at a green color
of around $545 \mu m$, and the S cones respond the most to short wave
length, peaking at a bluish color of around $450 \mu m$ \cite{Stockman_1993_vision}.
Colors of other wavelength will cause responses from the three types
of cones, allowing the brain to differentiate among different
colors. This also means that colors outside the response ranges of the
cones will be invisible to human eyes.


 If we consider
the intensity of each color as between 0 to 1, then the RGB color
space is the unit cube in 3D.
Assuming that a white background is used to draw the graph,
then we do not want edges to be very bright. Hence by default we use the RGB space
with $0 \le r,g,b \le 0.7$, assuming that 1 is the fully saturated color value.
Unless otherwise stated, all examples given in the paper are
resulted from applying CLARIFY in the RGB color space.

\subsection{LAB color space}

RGB color model is widely used for the representing and displaying
images in electronic systems, such as LCD/LED display. 
However, distance between two colors in the RGB space is not an accurate measure of
perceived difference by human eyes. For that purpose, 
the LAB color
model is consider better \cite{lab_color}.

The LAB color model is a three axis system that is device independent. The
 L axis stands for lightness and is between 0 to 100, the A axis 
goes from green to  magenta/red 
and the B axis goes from yellow to blue, both are between -128 to 128.
The LAB color space  is perceptually more uniform than RGB space, in the sense that
a change of the same amount in a color value should produce a change of 
about the same visual importance. 
The LAB color space includes all perceivable colors, and more.
When mapping RGB to LAB, the resulting gamut, hereafter referred to 
simply as the LAB color gamut, has a complex polygon like shape~(Fig.~\ref{lab}).
Mapping from RGB to LAB is unique, while that from LAB to RGB is not, due to
the fact that the number of colors representable by the LAB model exceeds that of the RGB color model,
and for a LAB color that is not representable in RGB, typically the closest RGB color is used for the mapping.

While we can use CLARIFY directly in the LAB color space, since eventually we need to 
render the resulting drawing on screen and in print, we need to convert the 
coloring to RGB. Therefore we need to work within the LAB color gamut.
Applying CLARIFY requires checking whether a cube is outside of the 
LAB gamut, which is considerablly more complicated than checking whether a point is outside of the gamut,
since we are not aware of an analytical closed-form expression of the LAB gamut. Instead we modify
CLARIFY slightly as follows. We first sample the LAB gamut: we subdivide L, A and B 
at one unit increment, and check whether the resulting points are inside the LAB gamut by converting
the point to RGB space, and backt to the LAB space. If the double-conversion ends at the same point (within
a threshold of 0.02 in Euclidean distance), the point is considered inside the LAB gamut. This resulted in 826816 points.
Note that we only have to find this sample set once and store as a file.
We then construct an octree over this point set. The CLARIFY algorithm using this
octree, without worrying about staying inside the LAB gamut. The sample technique also makes it very easy
to control the lightness of the color -- if we need to display the drawing in a dark background and
thus light colors are desired, we can simply filter out points with a low $L$ value in the sample.
Fig.~\ref{palette}~(f) shows the result of apply CLARIFY in the LAB space with $0\le L\le 70$, while
Fig.~\ref{palette}~(f) shows the result with $L\ge 80$ in a black background.

In terms of CPU time, we found that working in LAB space with the sampling technique gives
very similar CPU time to working in the RGB space. Speed can be further improved
if we take a coarser sample.

\begin{figure}[htbp]
\begin{center}
\includegraphics[height=5cm]{DATA/gamut_lab.jpg}
\end{center}
\caption{\small\textsf The complex shape of the LAB color gamut -- the part of the LAB color space that corresponds to the RGB color space.\label{lab}}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.33\linewidth]{DATA/lab_l25.jpg}\includegraphics[width=0.33\linewidth]{DATA/lab_l50.jpg}\includegraphics[width=0.33\linewidth]{DATA/lab_l75.jpg}
\end{center}
\caption{\small\textsf Cross section of the LAB color gamut at $L=25,50,75$. $x$-axes is ``A'' and $y$-axes is ``B''.\label{lab2}}
\end{figure}

\definecolor{darkgray}{gray}{0.05}
\begin{figure}[t]
\def\tabcolsep{1pt}
\begin{center}
\begin{tabular}{cc}
%\includegraphics[width=4.1cm]{DATA/karate_graphplot_color2.pdf}
\includegraphics[width=4.1cm]{DATA/karate_graphplot_color.pdf}
&\includegraphics[width=4.1cm]{DATA/karate_graphplot_color_lab.pdf}\\
(a) RGB
&(b) LAB ($0\le L\le 70$)\\
\includegraphics[width=4.1cm]{DATA/karate_graphplot_color_ColorBrewer_accent_8.pdf}
&\includegraphics[width=4.1cm]{DATA/karate_graphplot_color_ColorBrewer_dark2_8.pdf}\\
(c) ColorBrewer Accent\_8
&(d) ColorBrewer Dark2\_8\\
\fcolorbox{lightgray2}{darkgray}{\includegraphics[width=4.1cm]{DATA/karate_graphplot_color_ColorBrewer_pastel1_9.pdf}}
&\fcolorbox{lightgray2}{darkgray}{\includegraphics[width=4.1cm]{DATA/karate_graphplot_color_lab_l80.pdf}}\\
(e) ColorBrewer Pastel1\_9
&(f) LAB ($L\ge 80$)\\
\end{tabular}
\end{center}
\caption{\small\textsf Apply CLARIFY on the Karate graph in RGB, LAB color spaces, and using two ColorBrewer palettes. 
For (e) and (f), we used assume that a dark background is required. In (e)
a light pastel color palette is used, while in (f) we allows only LAB colors with intensity $> 80$.
\label{palettes}}
\end{figure}

\begin{comment}
~/CVSED/EDGE_COLORING/edge_distinct_coloring -color_scheme=ColorBrewer_dark2_8 DATA/karate_graphplot.gv | neato -n2 -Tpdf -Epenwidth=4 -Gbgcolor="#ffffff00" > DATA/karate_graphplot_color_ColorBrewer_dark2_8.pdf
~/CVSED/EDGE_COLORING/edge_distinct_coloring -color_scheme=ColorBrewer_accent_8 DATA/karate_graphplot.gv | neato -n2 -Tpdf -Epenwidth=4 -Gbgcolor="#ffffff00" > DATA/karate_graphplot_color_ColorBrewer_accent_8.pdf
~/CVSED/EDGE_COLORING/edge_distinct_coloring -color_scheme=lab DATA/karate_graphplot.gv | neato -n2 -Tpdf -Epenwidth=4 -Gbgcolor="#ffffff00" > DATA/karate_graphplot_color_lab.pdf
~/CVSED/EDGE_COLORING/edge_distinct_coloring -color_scheme=rgb DATA/karate_graphplot.gv | neato -n2 -Tpdf -Epenwidth=4 -Gbgcolor="#ffffff00" > DATA/karate_graphplot_color2.pdf
~/CVSED/EDGE_COLORING/edge_distinct_coloring -color_scheme=ColorBrewer_pastel1_9 DATA/karate_graphplot.gv | neato -n2 -Nfillcolor="#aaaaaa" -Npenwidth=2 -Ncolor="#ffffff" -Gbgcolor=black -Tpdf -Epenwidth=4 -Gbgcolor="#ffffff00" > DATA/karate_graphplot_color_ColorBrewer_pastel1_9.pdf
~/CVSED/EDGE_COLORING/edge_distinct_coloring -color_scheme=lab -lightness=80,100 DATA/karate_graphplot.gv | neato -n2 -Nfillcolor="#aaaaaa" -Npenwidth=2 -Ncolor="#ffffff" -Gbgcolor=black -Tpdf -Epenwidth=4 -Gbgcolor="#ffffff00" > DATA/karate_graphplot_color_lab_l80.pdf
\end{comment}



\subsection{User-define color palettes}

Any user defined color palette can be handled in a similar way to the LAB gamut -- we project the
color palette consists of $k$ colors from RGB space to the LAB space, then interpolate these $k$ colors to get
sufficient number of $K$ sample points.
We do so by subdividing the path linking these $k$ points in the LAB space into segments of equal distance.
The path can be based on natural ordering of the palette, or 
constructed as a shortest path by solving a Traveling Salesman Problem in 3D.
An octree is then constructed using the $K$ sample points and CLARIFY is applied over the octree.
Fig.~\ref{palettes} gives some examples of using the ColorBrewer~\cite{ColorBrewer2} color palettes, with $K = 10^4$.
Additional examples can be found at \url{http://www2.research.att.com/~yifanhu/EDGE_CLARIFY/}.



\subsection{Other color spaces}

There are situations where
other color space may be more appropriate. For example, for disambiguating 
the edges in Fig.~\ref{dual}, we avoided using colors for edges in order to 
accurately display colors of the nodes. For this drawing we used CLARIFY with the gray scale, so that edges are
in black or gray. We could even map the gray scale to
line styles, with black for solid line and gray for dashed line of different weights.




==> letter.tex <==

------------------------ Submission 340, Review 2 ------------------------

Title: A Coloring Algorithm for Disambiguating Graph and Map Drawings

Reviewer:          primary

Paper type

  Technique

Expertise

  2  (Knowledgeable)

Overall Rating

  2  (<b>Reject</b><br/> The paper is not ready for publication in InfoVis / TVCG.<br/>The work may have some value but the paper requires major revisions or additional work that are beyond the scope of the conference review cycle to meet the quality standard. Without this I am not going to be able to return a score of '4 - Accept'.)

Supplemental Materials

  Acceptable

Justification

  Interesting and useful idea to use color to help disambiguate edges
  during crossings, but my main concern is that this idea has been
  proposed and published elsewhere and thus the novelty and
  originality of this submission is significantly lessened. The work
  is therefore incremental, and is also burdened by minor issues with
  the statistical analysis of the user study results.

The Review

  This paper proposes an algorithm called CLARIFY to improve
  perception of incident edges for graph visualization using an edge
  coloring algorithm that will reportedly help the visual system
  disambiguate between the crossing lines. This idea is not new: it
  was originally proposed by Jianu et al. in a technique refered to as
  JRFL (cited as #26 in the paper). The stated contribution of this
  work is an improvement over the JRFL algorithm based on an entirely
  new algorithm and a better choice of edge colors. The work consists
  of in-depth algorithm descriptions, implementation notes, complexity
  analysis, and performance results. The algorithm is validated with a
  quantitative user study (N=12) comparing CLARIFY for node-level and
  edge-level graph tasks with a non-colored (black and white) graph.

  I was impressed by the elegance of this idea when I first read the
  abstract and intro: since edge crossings are a perceptual issue, we
  can find subtle ways to help human perception navigate them. More
  specifically, by coloring the offending edges in different ways, we
  can deal with the issue. However, it was only when I read further on
  in the paper that I realized that the authors were not the first to
  come up with this idea: it has already been published by Jianu et
  al. in a paper from IV 2009. While it is clear from the text that
  the authors only found this work after starting their own project, I
  still think the paper should be written so that this similarity is
  disclosed up front, i.e. already in the introduction of the work.

  So, at this point, reviewing this paper becomes all about
  determining the value of the proposed work (called CLARIFY) in
  comparison to that of Jianu et al. (refered to as JRFL).
  Understanding this, the authors spend considerable space comparing
  and discussing the differences and improvements in CLARIFY over
  JRFL. Furthermore, they devote a subsection to a qualitative
  comparison of the results of their algorithm with JRFL, finding that
  CLARIFY comes out on top. In addition, the JRFL paper only provided
  anecdotal findings showing that the idea is superior to non-colored
  graphs, whereas this submission presents a full-fledged user study
  that compared graph task performance with CLARIFY-colored graphs to
  uncolored graphs. Finally, there are certainly several good features
  in the CLARIFY algorithm that go beyond that of JRFL. In other
  words, there is clear merit to the contribution in this work.

  However, in the end, the IEEE InfoVis conference, in its position as
  the premier venue for information visualization work, values novelty
  and originality over algorithmic and methodological perfection. Even
  if this submission represents solid and useful research, it is still
  incremental in light of the literature in graph drawing, with the
  Jianu work essentially subsuming the idea. It is possible that an
  outright admission of the presence of the JRFL algorithm and a user
  study that formally compared CLARIFY graphs to JRFL graphs would
  have been more convincing. Anyway, for these reasons, I cannot
  recommend this paper for acceptance at IEEE InfoVis.

  Some additional minor points about the user study: As far as I can
  tell, the study has been conducted competently. However, I do not
  think that the task error analysis can be done using an ANOVA, since
  the 0 or 1 correctness is not a continuous metric. I would suggest
  using logistic regression, which is based on the binomial
  distribution. Second, the authors claim that some effects were
  significant, but only give p-values. It is customary to also provide
  F values with the nominator and denominator for the degrees of
  freedom (df, den) so that readers can assure themselves of the
  correctness of the analysis. 

  Another point is that the user study does not really provide any
  conclusive results other than the significant correctness
  improvement for connectivity analysis; I would have expected all of
  the tasks and not just the connectivity one to exhibit the positive
  effects of the coloring scheme. This leads me to believe that the
  study has not been calibrated properly to the point where
  demonstrable differences occur, and I would suggest the authors take
  the time to work on this if they are going to rerun the study with
  JRFL graphs as well anyway.

Summary Rating

  2  (<b>Reject</b><br/> The paper is not ready for publication in InfoVis / TVCG.<br/>The work may have some value but the paper requires major revisions or additional work that are beyond the scope of the conference review cycle to meet the quality standard. Without this I am not going to be able to return a score of '4 - Accept'.)

The Summary Review

  Reviewers all gave ratings on or below the neutral: two 3s, and two
  2s. Summarizing across reviews, all reviewers recognize that this is
  an interesting and potentially impactful idea that is based on
  features of the human visual system: if there are perceptual issues
  with coinciding and crossing edges, then we can use another
  perceptual aspect (color) to fix it. R1 think this is useful with
  medium to high impact, R2 thinks it is elegant, R3 calls it
  "interesting", and R4 echoes the usefulness and benefit of the
  technique. In addition, R4 notes that the paper is fairly complete
  and fits well the definition of an InfoVis technique paper.

  However, all reviewers raise two primary problems with the work:

  1. The dismissal of literature on k-colorability for graphs, which
      both R1 and R3 think are of key importance to the work; and

----
added discuss in related work on how this work and k-colorability is
related but different. The main difference is that in k-colorability
work, colors are considered distinict if they are different, i.e., the
distance of colors are binary -- 0 or 1. In this
work we want to maximize the color distances. If we only have
k-colors, then our algorithm effectively try to find the best
permutation of these colors.
---

  2. Comparisons with the earlier technique proposed by Jianu et al,
      which subsumes the innovation of this work (R1, R2, R3).

  Both R1 and R3, who are experts on this topic raise the first issue,
  and during discussions it was agreed that this is perhaps the most
  serious issue plaguing the paper. The paper does not acknowledge
  this body of work at all.

  As for the second issue, R2 and R3 are the strongest critics and
  thinks that even if the paper acknowledges the existence of the
  previous work, it may not be sufficient for an InfoVis submission.
  While all reviewers concede that the paper does provide evidence
  that the new technique is superior to that of Jianu et al., R2 in
  particular (i.e. me) argues that this is not enough, and that at the
  very least the Jianu algorithm should have been included in the
  evaluation.

  In the end, this paper is plagued with too many issues than can be
  reasonably considered a "minor revision". For this reason, I give a
  summary rating of 2 and recommend the paper be rejected.

Second round comments (public)


Second round supplementary materials check

  

Second round supplementary materials comments



------------------------ Submission 340, Review 1 ------------------------

Title: A Coloring Algorithm for Disambiguating Graph and Map Drawings

Reviewer:          secondary

Paper type

  Technique

Expertise

  3  (Expert)

Overall Rating

  3  (<b>Possible Accept</b><br/> The paper is not acceptable in its current state, but might be made acceptable with significant revisions within the conference review cycle.<br/>If the specified revisions are addressed fully and effectively I may be able to return a score of '4 - Accept'.)

Supplemental Materials

  Acceptable with minor revisions (specify revisions in The Review section)

Justification

  This paper presents a technique that uses color to disambiguate possibly
  colliding edges in a static representation of a graph. The authors
  outline the algorithm itself, its application to different types of
  problems and present the result of a small user study.

  Strengths
  - Potentially useful technique for static graphs, given it can also be
  used with other encodings.
  - Added user study adds to technique weight.

  Weaknesses
  - Only a cursory 2 line treatment of related research in Graph Coloring
  problems.
  - Seemingly overly complex color picking algorithm, with no rationale.

  I'm undecided. As is, the work is not acceptable, but could be adjusted
  to be acceptable with a few minor changes and one major change.

The Review

  This paper presents a technique that uses color to disambiguate possibly
  colliding edges in a static representation of a graph. The authors
  outline the algorithm itself, its application to different types of
  problems and present the result of a small user study.

  Impact is medium/high. This seems like an effective method to
  disambiguate edges, for simple connectivity estimation on static graphs.
  Authors also argue that the same method extends to any visual encoding,
  making the method broader than just color. Novelty is impacted by the
  prior publication of [26]. However, I think the authors have done a good
  job of contrasting their solution with the one presented in that paper,
  and have convinced me their solution is provably better. Using edge color
  to more clearly show connectivity is a relatively new idea.

  However, there is but a cursory reference in the related work to graph
  coloring problems, which the authors offhandedly dismiss saying that
  graph coloring does not consider maximizing difference on edges. Only to
  then immediately suggest computing the dual graph, and thus convert the
  problem back to a node coloring problem. Also, the maximum number of
  colors needed is known as at most 1+maxDegree (or just maxDegree, if you
  consider Brooks' theorem). Instead of incrementally adding colors while
  optimizing, couldn't you have computed a fixed set of 1+maxDegree
  maximally different colors first and then pick the two most distinct
  colors from that set? Instead authors use a fairly complicated
  incremental discrete optimization algorithm that will select colors from
  a large batch of potentials, where potentials are created by sampling the
  space or by interpolating a given palette. Do I really need 826816
  potential colors? Is it worth having the areas in Fig 9 each be a
  slightly different color?

  Another smaller technical issue is background color, which has been taken
  into account as dark vs light. Yes, the sample space could be reduces to
  only include high luminance or low luminance colors, but what if the
  background is grey? Would it have been an idea to also add background
  color to the color distance maximization?

  Finally, the user study shows the method works for connectivity
  estimation, but also shows increased task completion time (although not
  significantly) for path following tasks. I was expecting this, as the
  strong color cues may entice people to inadvertently follow a path of the
  same color. I would expect some discussion on this in the evaluation.

  Overall, I'm conflicted. Yes this is a potentially useful idea,
  especially if you also consider other encodings than color. Yes, this is
  an improvement over [26] but given some of the choices made there, that
  is not that hard. To be acceptable for IEEE Vis the following changes
  should be made:
  - Properly discuss graph coloring problems in the related work section.
  - Discuss the rationale for not simply picking maxDegree+1 colors in
  advance and using that as a fixed palette.
  - Discuss increased path following task completion time in section 5.
  - Add a sample of different encoding (e.g. line stipple).
  If ultimately found not to be acceptable, and obvious other choice is the
  GD conference.

  Other issues:
  - Please match colors between figure 2 and 4.
  - Merge section 6 and 7 into one.



------------------------ Submission 340, Review 3 ------------------------

Title: A Coloring Algorithm for Disambiguating Graph and Map Drawings

Reviewer:          external

Paper type

  Technique

Expertise

  3  (Expert)

Overall Rating

  2  (<b>Reject</b><br/> The paper is not ready for publication in InfoVis / TVCG.<br/>The work may have some value but the paper requires major revisions or additional work that are beyond the scope of the conference review cycle to meet the quality standard. Without this I am not going to be able to return a score of '4 - Accept'.)

Supplemental Materials

  Acceptable with minor revisions (specify revisions in The Review section)

Justification

  The authors show experimentally that there is benefit to colouring edges
  in graphs to resolve ambiguity.  Unfortunately, it appears they were
  unaware of similar work by Jianu while developing and evaluating their
  technique.  However, they argue and demonstrate at least on one graph
  that the technique by Jianu is inferior.
  I am concerned however, that they are also overlooking a wealth of
  literature on the k-colourability of graphs, for which fast greedy
  algorithms are already known.  I think they overlook this because they
  have focused on colouring using a continuous colour space.  However, in
  practice I think for reasons of taste you would want to use an extremely
  limited colour palette.  

The Review

  This is an interesting idea that stems from real need and it is explored
  by the authors both algorithmically and experimentally.  Similar work by
  Jianu [26] is cited and shown to be somewhate inferior.

  The proposed "collision" conditions given in 3.1 seem well reasoned. 
  However, it would be nice if they were supported by findings from the
  canon of perception.  Colin Ware's book surveys a lot of relevant
  material but there is probably more recent work if you look for it. 
  Also, in practice I think this technique would usually be applied
  together with an edge routing scheme that also tries to resolve edge
  ambiguity such as Pupyrev [30].  Given such a routing scheme what other
  criteria need to be considered?  At least the definition of "close
  parallel" edges would need to change to consider edges that can run
  parallel for some of the route and then diverge.

  In a real system I think I would always want to limit the colours used to
  a discrete pallette chosen in advanced to complement each other and other
  colours used in the UI.  The authors discuss this in Section 4.1, yet it
  seems crucial otherwise the results are just far too Jackson Pollock (I
  mean visually noisy and overwhelming).  In such a discrete optimization
  space, I wonder if the proposed algorithm is still really the best
  approach?  MIP or other general optimization methods should probably be
  employed before inventing new algorithms.

  Actually, given that in practice a very small number of colours is
  preferable, doesn't this become just a k-colouring problem of the
  edge-collision dual graph?  k-colourability is extremely well studied,
  with efficient greedy heuristics by Welsh-Powell, Brelaz etc.  For small
  graphs it can be solved optimally using dynamic programming.


------------------------ Submission 340, Review 4 ------------------------

Title: A Coloring Algorithm for Disambiguating Graph and Map Drawings

Reviewer:          external

Paper type

  Technique

Expertise

  2  (Knowledgeable)

Overall Rating

  3  (<b>Possible Accept</b><br/> The paper is not acceptable in its current state, but might be made acceptable with significant revisions within the conference review cycle.<br/>If the specified revisions are addressed fully and effectively I may be able to return a score of '4 - Accept'.)

Supplemental Materials

  Acceptable

Justification

  I think the paper is well written and that it contains most of the
  requirements for a technique paper (algorithm description and
  pseudo-code, complexity analysis, examples, running time, parameters used
  and user study). The technique can be useful in certain applications, and
  seems to be beneficial according to the results of the user study.
  However, I believe there are a few points to clarify before accepting the
  paper.

The Review

  The authors propose a method to improve the readability of graph edges
  using colours. Edges that risk to be misread, such as almost parallel
  edges, are assigned with different colours in order to remove the
  ambiguity. The colouring is said to be near-optimal, and the palette can
  be continuous or discrete, and defined in a space of arbitrary dimension.

  First, the authors introduce the problem and the related work. Then, they
  explain the techniques including details on the time complexity,
  parameters used, obtained results and comparison with existing
  techniques. Finally, they present a user study designed to evaluate the
  usefulness of the technique.

  I find the paper well written and well organised. The technique presented
  has its applications and uses a feature that is an established convention
  in certain diagrams (using colours to differentiate crossing lines is
  standard, for example, in metro maps). The algorithm seems to be
  sufficiently fast and flexible, and the colouring seems to have positive
  effects on the graph readability as shown in the user study.

  However, there are some points that I should be addressed before
  considering the paper acceptable:

  - I do not quite agree with the sentence "we believe that the idea of
  using colours to disambiguating edges is quite natural to think of". 
  When looking at Figure 1, I would think that the edge colours either
  encode a metric (edge weight), or define some grouping. I agree that
  colours work well after their real aim is explained, but this rationale
  hardly match the initial intuition.

  - In figure 1r, there seems to be a few problems with the colouring.
  According to the authors' explaination for nodes 19-20-17, condition 3
  should be enforced. However, nodes 1 and 20 are directly connected with a
  red edge, and indirectly connected through node 15 using blue edges. 
  These blue edges are almost parallel to the red line and therefore meet
  at node 15 at an angle of about 180°, yet they share the same colour.
  The same goes for 2-14-17 and 2-15-4.

  - Section 3. I would avoid using the term dual for the collision graph. A
  dual graph has a different established meaning and the collision graph
  does not have the symmetric property that motivates the word "dual": the
  dual collision graph of the dual collision graph is not the original one.

  - I think it would be possible to better explain the mechanism described
  in page 4, second column. A step by step image would greatly help.

  - It is not very clear to me if it is possible to use a custom palette of
  k colours, with colours pre-assigned, or if the method always requires
  the definition of a colour space. For example, is it possible to use the
  exact colours proposed by ColorBrewer for k data classes, or my own
  palette composed by three shades of green and one of blue? In the last
  case, would the method be able to recognise that the three shades of
  green are much closer to each other than they are with blue?

  - In section 5, I do not quite understand the scale used for "Task
  Error". What does a value of 1.5 mean?


  Minor comments:
  - page 2, about a quarter down the second column. "the idea of [...] are
  quite natural" -> "the idea of [...] is quite natural"
  - Figure 10 should be rescaled to better fit its column
  - Bibliography: entries 27 and 28 actually refer to the same publication


==> vgtc_journal_latex_13-vis/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> vgtc_journal_latex_13-vis/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

